Skeletal Representations and Applications

When representing a solid object there are alternatives to the use of traditional explicit (surface meshes) or implicit (zero crossing of implicit functions) methods. Skeletal representations encode shape information in a mixed fashion: they are composed of a set of explicit primitives, yet they are able to efficiently encode the shape's volume as well as its topology. I will discuss, in two dimensions, how symmetry can be used to reduce the dimensionality of the data (from a 2D solid to a 1D curve), and how this relates to the classical definition of skeletons by Medial Axis Transform. While the medial axis of a 2D shape is composed of a set of curves, in 3D it results in a set of sheets connected in a complex fashion. Because of this complexity, medial skeletons are difficult to use in practical applications. Curve skeletons address this problem by strictly requiring their geometry to be one dimensional, resulting in an intuitive yet powerful shape representation. In this report I will define both medial and curve skeletons and discuss their mutual relationship. I will also present several algorithms for their computation and a variety of scenarios where skeletons are employed, with a special focus on geometry processing and shape analysis.

==> extra.tex <==
% Extra medial properties
% \ignore{While interesting in theory, explicitly reconstructing the surface from a set of medial balls has not received broad interest in the literature because of the complexity associated with the superimposition operator}. On the other hand, the possibility of perfectly reconstructing the original shape from a set of medial balls has important consequences: any computation on the surface can be performed directly on the medial representation (see Ch.2 of~\cite{siddiqi_book09}).}

% SKIPPED Talk about thinning methods
One way of creating a volume loss is clearly by using a voxel-erosion process like the one used for medial axis computation, except that beyond homotopy we will have tests only for terminal points and none for sheet finding~\cite{svensson_prl02}\footnote{verify this reference}. 

% Multi-resolution
\cite{hilaga_sig01}: Multi-resolution Reeb-Graph by first extract high resolution then use adjacency rules to do collapses and create a coarse-to-fine representation. But how does it match???\\
\cite{cornea_tvc05} \\

% More on reeb
Extended Reeb-Graph [11,17,16] on \cite{biasotti_sas07}?? \\

% Growing blob
\textbf{Growing blob} \cite{sharf_eg07} using a deformable model which reconstruct the shape at the same time as extracting a centerline of the front.

%----------------------------------------------------------------------------%
%                             EPSILON SAMPLING
%----------------------------------------------------------------------------%
In order to be able to define the medial axis for Voronoi diagram we will need the notion of $\epsilon$-sampling~\cite{missing}. A \emph{sample} of the boundary of a shape $X$ is a finite set of points (precisely) on that boundary. An $\epsilon$-sample is a sample whose Hausdorff distance to the boundary of $X$ is less than $\epsilon$. A \emph{noisy} $\epsilon$-sample is a sample where the points are not restricted to the surface.

